Synergistic CPU-FPGA Acceleration of Sparse Linear Algebra

This paper describes REAP, a software-hardware approach that enables high performance sparse linear algebra computations on a cooperative CPU-FPGA platform. REAP carefully separates the task of organizing the matrix elements from the computation phase. It uses the CPU to provide a first-pass re-organization of the matrix elements, allowing the FPGA to focus on the computation. We introduce a new intermediate representation that allows the CPU to communicate the sparse data and the scheduling decisions to the FPGA. The computation is optimized on the FPGA for effective resource utilization with pipelining. REAP improves the performance of Sparse General Matrix Multiplication (SpGEMM) and Sparse Cholesky Factorization by 3.2X and 1.85X compared to widely used sparse libraries for them on the CPU, respectively.

==> background.tex <==
\section{Background}
This section provides a background on compressed sparse formats and sparse
generalized matrix multiplication.


\vspace{-2.5mm} 

\subsection{Compressed Storage Formats}
In many real-world applications, when a majority of a matrix's
elements are zeros that is referred to as a sparse matrix. The number
of non-zero elements divided by the total number of elements in the
matrix is termed as the \textit{density} of the matrix.


\begin{figure}[t!]
  \centering
  \includegraphics[width=0.5\textwidth]{figures/sparseformat.pdf}
  \caption{\small Two common sparse format representations. a) A dense
    representation of the matrix b) A sparse COO representation of the
    matrix c) A sparse CSR representation of the matrix}
  \label{fig:sparse_formats}
\end{figure}


It is inefficient to use the same storage format for a sparse matrix as for a dense one.
Researchers have suggested different compression schemes to
avoid storing zero elements \cite{Bader:cooformat}
\cite{Buluc:dcsr}\cite{Saad:csr}\cite{Kincaid:ellpack}. Each of these
sparse formats is ideal under certain conditions; there is not a
superior format to store sparse matrices. The ideal format depends on
different metrics such as the sparsity pattern, the computation, and the
hardware used. It is thus desirable if multiple formats are supported,
otherwise, extra formatting is required to put the data into the
supported format.  The two commonly sparse formats are the compressed
sparse row (CSR) format and the coordinate format (COO). Figure
\ref{fig:sparse_formats} illustrates the way these two formats store
the non-zero elements of a matrix.

\textbf{Coordinate format (COO).} One simple way to store a sparse
matrix is to keep a list of the nonzero values combined with their
corresponding coordinates (\ref{fig:sparse_formats}.b). This is known
as the coordinate (COO) format.

\textbf{Compressed sparse row (CSR).}  The COO format redundantly
stores row coordinates for every nonzero value. One way to remove
storing this redundant row coordinates is by using an auxiliary array
that keeps track of which non-zeros belong to each row. The values and
columns of the nonzero elements are stored row by row in the two
separate arrays. Then we store the starting offsets for all the rows
in another array, commonly name \textit{row\_pointer} array. This
method of storing the nonzero values is called Compressed Sparse Row
(CSR) \ref{fig:sparse_formats}.c. The dual of CSR format is called
Compressed Sparse Column (CSC) that the column pointers are kept
instead of the rows and the nonzero values are stored in column-major
fashion in contrast to a row-major fashion in CSR format.
\vspace{-2.5mm} 
\subsection{Sparse General Matrix Multiplication}
One of the sparse kernels we study in this work is Sparse General
Matrix Multiplication is commonly known as SpGEMM. In SpGEMM, we multiply
two sparse matrices A and B which results in another sparse matrix
(C).  There are different algorithms to perform SpGEMM which are
inspired by the algorithms for general matrix-matrix multiplication in
a dense setting. These algorithms are different in the way they access
the input matrices and the order the output is produced. In general,
there are four formulations as shown in Figure~\ref{fig:spgemm} to
compute SpGEMM.
\begin{enumerate}
\item \textbf{Row by column} (known as inner product) In this method,
  for each row of matrix A, we calculate a dot product with all the
  columns of matrix B (Figure~\ref{fig:spgemm}.a).
\item \textbf{Column by column} For each column of B, we multiply each
  column of A, one column at a time(Figure~\ref{fig:spgemm}.b )
\item \textbf{Row by Row} Each row of A is multiplied with each row of
  B one at a time (Figure~\ref{fig:spgemm}.c)
\item \textbf{Column by row} (known as outer product) In contrast to
  the inner product method, the outer product takes each column of A
  and a row of B and do the outer product of the two vectors
  (Figure~\ref{fig:spgemm}.d)
\end{enumerate}


\begin{figure}[t!]
  \includegraphics[width=0.5\textwidth]{./figures/spgemm.pdf}
  \caption{\small Four different formulations to do General Matrix
    Multiplication a) The inner product b) The column by column method
    c) The row by row method d) The outer product}
  \label{fig:spgemm}
\end{figure}

Choosing the right algorithm for sparse kernels is a challenging job
and depends on many factors including the sparse format the inputs
were given, the memory and the computational features of the system
you execute are the most important factors in choosing the right
algorithm \cite{Zhen:IA-SOGEMM:ICS:2019}.
%


This paper adopts the row-by-row method for our SpGEMM
design~(Section~\ref{spgemm-detail}), which is also used by Intel Math
Kernel Libraries (MKL).









==> designdetails.tex <==
\input{spgemm.tex}

\input{cholesky.tex}

\input{hardware.tex}


==> motivation.tex <==
\section{Motivation}

Two points we want to explain here. 

First, why sparse format adds challenges 

One there exist inefficiencies from the computation perspective. In
any sparse format, there is a separation between the actual data and
the position of the data in the original matrix.  The downside of this
separation is, to access a non-zero value, first, you have to locate
it in the data array. The overhead results from this extra lookup are
mainly three folds. One, this lookup adds extra instruction and as a
result, extra cycle to the computation. Two, there is a side effect
for these additional instructions such as cache pollution, extra
memory traffic that can adversely affect performance. There is a
recent study that shows that in an ideal scenario, where accessing the
none-zero elements does not incur any cost, the performance of the
Sparse Matrix Multiplication can be improved almost 3 times. Three,
all the indirect data-dependent accesses, make little room for any
compiler-level optimizations that will commonly use to improve the
performance of the kernel in a dense setting. Figure [] shows the
CSR-based an inner product implementation of SpGEMM where both inputs
are in CSR format. As you can see in the figures, the non-zeros should
be extracted first at lines[], before any computation should take
place. These accesses incur a lot of overheads.

Second, why using the FPGA for the computation 
Use some text and figures from the NSF proposal. 





